A Unified Treatment of Partial Stragglers and Sparse Matrices in Coded Matrix Computation

The overall execution time of distributed matrix computations is often dominated by slow worker nodes (stragglers) within the clusters. Recently, different coding techniques have been utilized to mitigate the effect of stragglers where worker nodes are assigned the job of processing encoded submatrices of the original matrices. In many machine learning or optimization problems the relevant matrices are often sparse. Several prior coded computation methods operate with dense linear combinations of the original submatrices; this can significantly increase the worker node computation times and consequently the overall job execution time. Moreover, several existing techniques treat the stragglers as failures (erasures) and discard their computations. In this work, we present a coding approach which operates with limited encoding of the original submatrices and utilizes the partial computations done by the slower workers. While our scheme can continue to have the optimal threshold of prior work, it also allows us to trade off the straggler resilience with the worker computation speed for sparse input matrices. Extensive numerical experiments done in AWS (Amazon Web Services) cluster confirm that the proposed approach enhances the speed of the worker computations (and thus the whole process) significantly.

==> bio.tex <==

\begin{IEEEbiographynophoto}{Anindya Bijoy Das}
(das207@purdue.edu) is currently a postdoctoral researcher at Department of Electrical and Computer Engineering in Purdue University, West Lafayette, IN 47907 USA. 
He completed his PhD and M.Engg. from the Department of Electrical and Computer Engineering at Iowa State University in 2022 and 2018, respectively. He received his B. Sc. degree in Electrical and Electronic Engineering from Bangladesh University of Engineering and Technology, Dhaka, in 2014. His research interests include federated learning, coding theory and machine learning. He is the recipient of the Karas Award 2022 in Iowa State University for his outstanding thesis in the area of Mathematical and Physical Sciences and Engineering. He also received research excellence and teaching excellence awards from the Department of Electrical and Computer Engineering at Iowa State University.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Aditya Ramamoorthy}
 (adityar@iastate.edu) is a Professor of Electrical and Computer Engineering and (by courtesy) of Mathematics at Iowa State University. He received his B. Tech. degree in Electrical Engineering from the Indian Institute of Technology, Delhi and the M.S. and Ph.D. degrees from the University of California, Los Angeles (UCLA). His research interests are in the areas of classical/quantum information theory and coding techniques with applications to distributed computation, content distribution networks and machine learning.

Dr. Ramamoorthy served as an editor for the IEEE Transactions on Information Theory from 2016 — 2019 and the IEEE Transactions on Communications from 2011 — 2015. He is the recipient of the 2020 Mid-Career Achievement in Research Award, the 2019 Boast-Nilsson Educational Impact Award and the 2012 Early Career Engineering Faculty Research Award from Iowa State University,  the 2012 NSF CAREER award, and the Harpole-Pentair professorship in 2009 and 2010. He is a senior member of the IEEE.
\end{IEEEbiographynophoto}
